Quantum Filter Diagonalization with Double-Factorized Hamiltonians

We demonstrate a method that merges the quantum filter diagonalization (QFD) approach for hybrid quantum/classical solution of the time-independent electronic Schr\"odinger equation with a low-rank double factorization (DF) approach for the representation of the electronic Hamiltonian. In particular, we explore the use of sparse "compressed" double factorization (C-DF) truncation of the Hamiltonian within the time-propagation elements of QFD, while retaining a similarly compressed but numerically converged double-factorized representation of the Hamiltonian for the operator expectation values needed in the QFD quantum matrix elements. Together with significant circuit reduction optimizations and number-preserving post-selection/echo-sequencing error mitigation strategies, the method is found to provide accurate predictions for low-lying eigenspectra in a number of representative molecular systems, while requiring reasonably short circuit depths and modest measurement costs. The method is demonstrated by experiments on noise-free simulators, decoherence- and shot-noise including simulators, and real quantum hardware.

==> piece.tex <==
To describe the circuit reductions allowed by the combination of QFD and DF, we express the Hamiltonian as in Eq.~\eqref{eq:df_hamiltonian},
\begin{equation}
\begin{split}
\hat{H} 
&= 
E_{\mathrm{Ext}}
+
\sum_{k}
f_{kk}^{0}
\hat E_{kk}^{+}(0)
+
\sum_{t}
\sum_{kl}
\frac{ Z_{kl}^{t} }{2}
\hat E_{kk}^{+}(t)
\hat E_{ll}^{+}(t) \\
&= 
E_{\mathrm{Ext}}
+
\changeofbasis{0}{\mathrm{hf}}
\left[ \sum_{k \sigma}
f_{kk}^{0}
\numberop{k,\sigma}
\right]
\changeofbasis{\mathrm{hf}}{0} \\
&+ 
\sum_t
\changeofbasis{t}{\mathrm{hf}}
\left[ \sum_{kl,\sigma\tau}
\frac{ Z_{kl}^{t} }{2}
\numberop{k,\sigma}
\numberop{l,\tau}
\right]
\changeofbasis{\mathrm{hf}}{t}
\end{split}
\end{equation}
Here, $\changeofbasis{\mathrm{hf}}{l}$ denotes a unitary transforming from the Hartree-Fock basis to the 
eigenbasis of the $l$-th term of the Hamiltonian.
The index $l=0$ represents the the 1-body term,
and the indices $l=1 \dots \nlayers$ represent the
terms of the double factorized Hamiltonian.

Under the Jordan-Wigner mapping, number operators 
$\numberop{k,\sigma}$ and products of number 
operators $\numberop{k,\sigma} \numberop{l,\tau}$
take the form
\begin{equation}
\begin{split}
\numberop{k,\sigma}
&=
\frac{\left(1-Z_{k,\sigma}\right)}{2} 
\\
\numberop{k,\sigma}
\numberop{l,\tau}
&=
\frac{\left(1-Z_{k,\sigma}\right)}{2} 
\frac{\left(1-Z_{l,\tau}\right)}{2} 
\end{split}
\end{equation}
As seen, products of number operators contain terms 
that are linear in $Z_{k,\sigma}$. Our goal is to re-organize the Hamiltonian into a new one-body part
and a set of two-body factors involving only products
of the form $Z_{k,\sigma} Z_{l,\tau}$.
To this purpose, we introduce the operators
$\zetaop{k,\sigma} = 1-2 \numberop{k,\sigma}$ and
recall that $\zetaop{k,\sigma}^2 = 1$, we can 
readily recast Eq.~\eqref{eq:df_hamiltonian} 
in the form
\begin{equation}
\begin{split}
\hat{H} 
&= 
E_{\mathrm{Ext}}^\prime
+
\changeofbasis{0}{\mathrm{hf}}^\prime
\left[ \sum_{k \sigma}
f_{kk}^\prime
\,
\zetaop{k,\sigma}
\right]
\changeofbasis{\mathrm{hf}}{0}^\prime \\
&+
\sum_t
\changeofbasis{t}{\mathrm{hf}}
\left[ \sum_{kl,\sigma\tau}^*
\frac{ Z_{kl}^{t} }{8}
\zetaop{k,\sigma}
\zetaop{l,\tau}
\right]
\changeofbasis{\mathrm{hf}}{t}
\end{split}
\end{equation}
where the asterisk denotes summation over 
strings $kl,\sigma\tau$ with $k \neq l$, 
or $k=l$ and $\sigma \neq \tau$, and primes
denote a simple redefinition of the Hamiltonian coefficients and of the unitary transforming
from the Hartree-Fock basis to the eigenbasis
of the one-body part of the Hamiltonian.

In this form, time evolution under the Hamiltonian
for a time step $\Delta t$ can be approximated by
\begin{equation}
\label{eq:df_hamiltonian_circuit}
\hat{U}_{\Delta t}
\simeq 
e^{- i \Delta t E_{\mathrm{Ext}}^\prime}
\,
\changeofbasis{\nlayers}{\mathrm{hf}}
\left[
\prod_t 
\hat{V}_{\mathrm{2b},t} 
\,
\changeofbasis{t-1}{t}
\right]
\hat{V}_{\mathrm{1b}} 
\,
\changeofbasis{\mathrm{hf}}{0}^\prime
\end{equation}
where 
\begin{equation}
\begin{split}
\hat{V}_{\mathrm{1b}} 
&=
\prod_{k,\sigma}
e^{ - i \Delta t f_{kk}^\prime \, \zetaop{k,\sigma}}
\quad, \\
\hat{V}_{\mathrm{2b},t}
&=
\prod_{kl,\sigma\tau}^*
e^{ - i \Delta t \frac{ Z_{kl}^{t} }{8}
\zetaop{k,\sigma}
\zetaop{l,\tau} }
\quad,
\end{split}
\end{equation}
and 
$\changeofbasis{t-1}{t} = \changeofbasis{t-1}{\mathrm{hf}}
\changeofbasis{\mathrm{hf}}{t}$.

In this form, each of the change-of-basis unitaries $\hat{G}$ factors in two identical parts, acting on spin-up and spin-down spin-orbitals respectively. 
Such parts can be compiled into networks of Givens rotations, which can in turn be represented with 
one- and two-qubit gates, as discussed in the 
Appendix.
Furthermore, in the Jordan-Wigner representation,
evolution under the one-body part of the Hamiltonian
can be implemented by a network of single-qubit $Z$ rotations, and each of the terms
$\exp\left(-i \,\Delta t \, Z^t_{kl} \, \zetaop{k,\sigma} \,
\zetaop{l,\tau} \right)$ can be implemented with
2 \cnot and and single $Z$ rotation, as discussed 
in the Appendix.

\begin{figure}
\includegraphics[width=\columnwidth]{circuits/figures-figure1.eps}
\caption{Quantum circuit implementing time evolution under the DF Hamiltonian for a time step $\Delta t$. Green, red and orange blocks denote change-of-basis unitaries, evolution under diagonal one-body, and evolution under diagonal two-body operators respectively, and 
violet lines denote echo unitaries parametrized by angles $\eta_k$.}
\label{fig:qfd_2}
\end{figure}

The quantum circuit implementing the controlled 
version of the unitary transformation Eq.~\eqref{eq:df_hamiltonian_circuit} is shown
in Fig.~\ref{fig:qfd_2}.
It is useful to observe that unitaries $\hat{G}$ 
multiply to the identity and thus, as seen in 
Fig.~\ref{fig:qfd_2}, they need not be controlled.
In the Jordan-Wigner representation, each 
controlled $\exp\left( - i \Delta t \, f_{kk}^\prime 
\, \zetaop{k,\sigma} \right)$ can be constructed
with 2 \cnot and 2 $R_z$ gates, whereas each
controlled $\exp\left(-i \,\Delta t \, Z^t_{kl} \, \zetaop{k,\sigma} \,
\zetaop{l,\tau} \right)$ by 
4 \cnot and 2 $R_z$ gates.
